Exploring the Role of Social Support when Integrating Generative AI into Small Business Workflows

Small business owners stand to benefit from generative AI technologies due to limited resources, yet they must navigate increasing legal and ethical risks. In this paper, we interview 11 entrepreneurs and support personnel to investigate existing practices of how entrepreneurs integrate generative AI technologies into their business workflows. Specifically, we build on scholarship in HCI which emphasizes the role of small, offline networks in supporting entrepreneurs' technology maintenance. We detail how entrepreneurs resourcefully leveraged their local networks to discover new use cases of generative AI (e.g., by sharing accounts), assuage heightened techno-anxieties (e.g., by recruiting trusted confidants), overcome barriers to sustained use (e.g., by receiving wrap-around support), and establish boundaries of use. Further, we suggest how generative AI platforms may be redesigned to better support entrepreneurs, such as by taking into account the benefits and tensions of use in a social context.

==> Paper_Content/1.1_IntroductionOLD.tex <==
%==================================================================
% From this exploratory study, this short paper then also contributes a set of design implcations for future work which support the social context around generative AI, highlighting the importance of meeting entreprenuers where they are at through familiar platforms, taking into account the emergent social tensions arise in shared generative AI systems, and providing simple affordances (e.g. large buttons to facilitate exploration) that go beyond chat interfaces to overcome challenges with prompting.

% Specifically, this paper highlights the significance of local networks in not only adopting new technologies but also in shaping their usage in a way that respects their social, ethical, and practical boundaries.
% \yasmine{method details?}
% Ultimately, these insights pave the way for future work aimed at designing generative AI tools that are more attuned to the complex socio-technical milieu surrounding entrepreneurship.

% 


%; specifically in one city known for its post-industrial resiliency and strife, Pittsburgh, Pennsylvania.
% where economic mobility opportunities are limited and entrepreneurship serves to address socioeconomic divides.
% In particular, this paper details entreprneuers' resourceful tactics for sustaining use by leveraging trusted peers to overcome the myriad technical challenges to adopting generative AI.


% ======================== DEADHEADING  ========================


% When incorporating generative AI tools entrepreneurs must  navigate issues surrounding privacy and IP and copyright when inputting to and receiving output from generative models.
% Beyond prompt engineering, entrepreneurs must master many other computing skills to successfully integrate generative AI technologies into business workflows such as understanding file types and file conversions, word processing software skills to refine generated text, and graphic design knowledge to edit images, among others~\cite{kotturi2024deconstructing}.

% In addition, given that generative AI technologies are largely designed for individual use, we ask:
% \textbf{RQ2: How can generative AI platfroms be designed to support social use of generative AI technologies?}


% Moreover, local entrepreneurs must navigate factual inaccuracies in generated content \cite{10.1162/tacl_a_00324} alongside new interaction paradigms for generative models \cite{morris2023design}, further complicating the adoption generative AI into business practices.
% Small business owners who effectively leverage generative AI for their business can boost their efficiency and creativity, and ultimately increase their bottom line \cite{Otis2023UnevenImpact}.
% Entrepreneurs from lean economies, who primarily target their local economy and have small-scale product or service businesses (i.e., ``local entreprenuers'' \cite{10.1145/3313831.3376363})---may be uniquely positioned to reap the benefits of distributing tasks to a generative AI assistant given limited resources \cite{genAIworkshops}.
% Yet, to date, users of generative AI tools like ChatGPT have largely been limited to those who are college-educated or have technical backgrounds \cite{pew-research}.
% And while local entrepreneurs' backgrounds are expansive and not monolithic, human-computer interaction (HCI) scholarship has detailed at length the challenges of digital engagement among local entrepreneurs, such as skill barriers, lack of trust, heightened risk given connection to livelihood, and the constant self-upgrading and technical maintenance required to keep pace i.e. the ``additional labors'' of digital engagement~\cite{10.1145/3173574.3173814, avle2019additional, 10.1145/3313831.3376363, 10.1145/3274340, 10.1145/3313831.3376587, 10.1145/3449089}.% In this short paper, we build on this body of scholarship by considering the challenges with adoption and sustained use of generative AI technologies among local entrepreneurs.
% % , in light of disparities in use and the unique difficulties of keeping up with a rapidly evolving technology.
% To overcome these challenges with digital engagement, local entrepreneurs turn to small, local networks for vetted and trustworthy information of which digital tools to use, and for social support~\cite{10.1145/3313831.3376363,10.1145/3491102.3517708, 10.1145/3491102.3501949}. 
% % In addition Kotturi \textit{et al.} presented a model of personalized support which tailored technical advice to entrepreneurs' unique business domains, interests, and resources
% % \cite{10.1145/3491102.3517708}.




% \section{Introduction}
% % this feels so awkward, i think it's happening around sentence 3, and the first sentence is short and not enticing.....
% Generative AI has demonstrated its potential to have a transformative impact on the workplace \cite{mckinsey-report, eloundou2023gpts}. 
% Entrepreneurs who can effectively incorporate generative AI into their business stand to gain by increasing efficiency \cite{Peng2023ImpactOfAIDeveloper}, augmenting creativity \cite{Doshi2023GenerativeAI}, improving the quality of their output \cite{Girotra2023IdeasAD}, and ultimately increasing their bottom-line \cite{Otis2023UnevenImpact}.
% However, local entrepreneurs, who primarily target their local economy, often lack infrastructural support for technology adoption, and are thus especially vulnerable to the widening digital divides \cite{bbc-digital-literacy} brought on by generative AI.
% Beyond the vast array challenges local entrepreneurs must overcome during technology adoption \cite{10.1145/3173574.3173814, 10.1145/3359320, 10.1145/3313831.3376363, 10.1145/3274340, 10.1145/3313831.3376587, 10.1145/3449089, 10.1145/3449089}, legal uncertainties surrounding intellectual property \cite{mitsloan-generative-ai}, factual inaccuracies in generated content \cite{10.1162/tacl_a_00324}, and new interaction paradigms for generative models \cite{morris2023design} further complicate adopting generative AI into business practices. 
% While recent work in HCI highlights the importance of social support for local entrepreneurs to overcome these challenges when onboarding to generative AI technologies \cite{genAIworkshops}, there remains a gap in understanding how, after onboarding, local entrepreneurs continue to address these challenges to sustain their use. This paper aims to shed light on this area.

% Therefore, building off prior scholarship that shows how local entrepreneurs leverage their local network when acquiring new tech-skills \cite{10.1145/3313831.3376363, 10.1145/3491102.3501949, 10.1145/3359320}, we conducted a Speed Dating \cite{ZIMMERMAN201730} study with local entrepreneurs and support providers, guided by two main research questions:


% % \yasmine{Small local networks are important when acquiring tech skills for local entrepreneurs, therefore we ask:}

% \begin{itemize}
%     \item \textbf{RQ1}: How do small local networks facilitate, sustain, and impede local entrepreneurs' use of generative AI technologies?
% \end{itemize}

% Given that generative AI technologies are largely designed for individual use, yet local entrepreneurs benefit from social support when using technology, we ask:

% \begin{itemize}
%     \item \textbf{RQ2}: How can technology be designed to support social use of generative AI technologies?
% \end{itemize}

% % Our analysis revealed that entrepreneurs form small local networks for shared use of generative AI through shared accounts, encompassing trusted individuals such as family members, business partners, and peers from in-person incubators. 
% Our analysis revealed that entrepreneurs, through trusted peers, incubators, and small business workshops, relied on their small local networks for their introduction and continued use of generative AI technologies.
% Despite the single user design of these tools, entrepreneurs appropriated existing systems for shared use (e.g. sharing accounts) to overcome operational barriers, like prompting, to using generative AI and build self-efficacy.
% % These networks serve as sources of discovery, showcasing the diverse applications of generative AI, and as mediators, helping to refine requests and ensure practical outputs. 
% We observe that sharing use of the technology was critical to keep up with the pace of innovation: entrepreneurs who had the richer, continuous support that shared use affords tended to have more sustained use of generative AI beyond introductions.
% Additionally, we observe that local entrepreneurs establish boundaries in their adoption of generative AI, delineating ethical, and sometimes socially construed, boundaries of use, like that between art and business centered tasks. 
% Last, we provide initial implications for designing tools supporting social uses of generative AI among entrepreneurs, highlighting the importance of meeting entrepreneurs where they are at through familiar platforms, the dangers of model-centric solutions to providing support, and simple affordances that go beyond chat interfaces to overcome challenges with prompting.

% Overall, this research contributes rich empirical data provide an understanding of how local entrepreneurs navigate the burgeoning field of generative AI through an exploratory Speed Dating study with seven local entrepreneurs and four technical providers in the [Removed for Anonymity] area. 
% % Specifically, this paper highlights the significance of local networks in not only adopting new technologies but also in shaping their usage in a way that respects their social, ethical, and practical boundaries.
% Ultimately, these insights pave the way for future work aimed at designing generative AI tools that are more attuned to the complex socio-technical milieu surrounding entrepreneurship.
% % ==========================================













% % and but therefore

% % more definitional work --> what are these terms?

% % Entrepreneurship in the digital age has largely been hailed as a driver for innovation, economic mobility, and social change \cite{10.7551/mitpress/2333.001.0001}. 
% % % \yasmine{[one sentence - what is digital entrepreneurship?]}
% % % Digital entrepreneurship, which is characterized by the use of various electronic means to engage in business \cite{digital-entrepreneurship}, has become a prevalent feature of other types of 21st-century entrepreneurship through the rise of social, e-commerce, and mobile platforms.
% % Yet, scholars have questioned the perception of digital entrepreneurship as a ``democracatizing'' force \cite{10.7551/mitpress/2333.001.0001}, surfacing how the constant self-upgrading and technical maintenance required for entrepreneurs to stay relevant disproportionately disadvantages under-resourced and non-technical entrepreneurs \cite{10.1145/3359320, 10.1145/3274340} -- worsening existing digital divides \cite{bbc-digital-literacy, 10.1145/2858036.2858343}. 
% % % \yasmine{local entrepreneurship? define and tie in}
% % Local entrepreneurs, who target their local economy \cite{10.1145/3313831.3376363}, are especially vulnerable to these digital divides due to the economic limitations arising from their geographic scope.

% % However, given the myriad of ethical \cite{10.1145/3544549.3585657} and technical challenges \cite{10.1145/3544548.3581388} pertinent to entrepreneurial adoption of generative AI, it is unclear how local entrepreneurs utilize these networks in the context of generative AI. This paper aims to shed light on this area.












% % ============= V2 =============
% % \section{Introduction}
% % Entrepreneurship in the digital age has largely been hailed as force for innovation, economic mobility, and social change \cite{10.1145/3274340}. However, scholars have brought these notions into question, surfacing how the constant self-upgrading and technical maintenance required for entrepreneurs to stay relevant disproportionately disadvantages under-resourced and non-technical entrepreneurs \cite{10.1145/3359320} --- worsening existing digital divides \cite{bbc-digital-literacy}. Prior scholarship has made light on how entrepreneurs leverage peer networks for 


% % Prior scholarship highlights entrepreneurs engage peers to meet the demands of digital age \cite{}. From feedback seeking on social media to blah blah for blah blah. 

% % Recently, generative AI technologies have garnered attention for their transformative impact on the workplace \cite{mckinsey-report, eloundou2023gpts}, demonstrating increased efficiency, augmented creativity, and improved worker output associated with it's use \cite{Doshi2023GenerativeAI, Girotra2023IdeasAD, Peng2023ImpactOfAIDeveloper}. Though the causal effects of generative AI on entrepreneurial performance remain unclear \cite{Otis2023UnevenImpact}, the hype-driven rhetoric surrounding the technology and it's initial promise create a uniquely high pressure to adapt or be left behind. At the same, legal uncertainties surrounding intellectual property \cite{mitsloan-generative-ai}, factual inaccuracies in generated content \cite{10.1162/tacl_a_00324}, and new interaction paradigms for generative models \cite{morris2023design} further complicate adopting generative AI into business practices. Given the myriad of ethical and technical challenges pertinent to entrepreneurial adoption of generative AI, it is unclear how local entrepreneurs utilize these networks in the context of generative AI. This paper aims to shed light on this area.
% % % ---------

% % Therefore, we conducted a Speed Dating \cite{ZIMMERMAN201730} study with  local entrepreneurs and support providers, guided by two main research questions: \textbf{RQ1}: Small local networks are important when acquiring tech skills for local entrepreneurs, what do these small local networks look like, and how do they facilitate and/or impede use of generative AI technologies? \textbf{RQ2}: How can technology be designed to support social use of generative AI technologies?

% % Our analysis revealed that entrepreneurs form small local networks for shared use of generative AI through shared accounts, encompassing trusted individuals such as family members, business partners, and peers from in-person incubators. Despite the individual-centric design of these tools, the communal approach to their use is critical to keeping up with the pace of innovation. These networks serve as sources of discovery, showcasing the diverse applications of generative AI, and as mediators, helping to refine requests and ensure practical outputs. Additionally, we observe that local entrepreneurs establish boundaries in their adoption of generative AI, delineating social, ethical, and practical parameters to guide its use. Last, we provide initial implications for designing tools supporting social uses of generative AI among entrepreneurs.

% % Overall, this research contributes to a deeper understanding of how local entrepreneurs navigate the burgeoning field of generative AI. It highlights the significance of local networks in not only adopting new technologies but also in shaping their usage in a way that respects social, ethical, and practical boundaries. Ultimately, these insights pave the way for future work aimed at designing generative AI tools that are effective and attuned to the varied landscapes of entrepreneurial innovation.

% % maybe i need something justifying the second question more; like current technologies don't surround the use of social support;
% %       - gen AI is a collaborator
% %       -  while entreprenuers engage in peer-feedback for other things in the ideation process 
% %  generative AI as a collaborator in certain entreprenuership processes;
% % the current design of generative AI technologies doesn't revolve around these collaborative processes
% % there is a framework for this -- i just forget the paper (but the creative writing x generative AI paper, does look at it)








% % Prior scholarship in human-computer interaction (HCI) investigates various ways in which local entrepreneurs from lean economies 
% % % here, kotturi, dillahunt, hui;

% % While these models for social support 

% % Prior work shows the role of peer support in ---, ---, and ----. This authors shows how entrpeenures utilize feedback for -----. While --- expands on this by showing how entreprenurs ----. Alas,



% % Prior scholarship has shown how local entrepreneurs - who aim to serve their local economy - rely on their local networks in


% % From Otis et al 2023:
% % Consistent with the optimism currently surrounding generative AI (AI hereafter), recent experiments show that conversing with and receiving AI assistance causes workers to write faster  and  better  business  text,  including  press  releases,  ad  copy,  consulting  memos,  and customer support messages (Brynjolfsson, Li, and Raymond, 2023; Dell’Acqua et al., 2023;Doshi and Hauser, 2023; Noy and Zhang, 2023; Chen and Chan, 2023).



% % Prior scholarship studying how local entrepreneurs - who aim to serve their local economy - from lean economies leverage their local networks when acquiring technical skills by engaging community resources, peers, and tech capacity building programs \cite{}. However, it remains unclear how local entrepreneurs leverage these networks in navigating the landscape of generative AI. In this study we ask the following questions:

% % Yet, how entrepreneurs, particularly those from low-tech backgrounds, adopt generative AI technologies remains unclear. Further, HCI researchers have highlighted how current interaction paradigms for generative AI (e.g. prompting) are not conducive to non-expert users.
% % I don't like this sentence.
% % \begin{enumerate}
% %     \item Small local networks are important when acquiring tech skills for local entrepreneurs, what do these small local networks look like, and how do they facilitate and/or impede use of generative AI technologies?
% %     \item Further, how can technology be designed to support social use of generative AI technologies?
% % \end{enumerate}

% % In this paper we present the empirical findings from a Speed Dating \cite{ZIMMERMAN201730} study with seven local entrepreneurs and four providers of entrepreneurship support in the greater [CITY] area. We find that even though use is designed for the individual, entrepreneurs assemble small local networks to use generative AI through shared accounts, entrepreneurs establish social, ethical, and economic boundaries of use. Further we present initial implications for designing technology to support entrepreneurs in using generative AI. 







% % Technical Barriers with up-keep.
% % Prior work studying how local entreprneurs overcome these technical barriers relying on their local networks through peers, community, tech-capacity building.

% % Recently, Discussion around generative AI and its impact on workplace performance. Studies showing increased efficiency with generative AI in the firm. Despite this, entreprenuers leveraging generative AI have to deal with a range of complexity unseen with other technologies, such as ethical issues with ownership, IP, humanity (with art? what does art mean, what does it mean to be human?) hallucinations, fast-pace and hype driven rhetoric, At the same time HCI research has shown how the interaction paradigms for generative AI technologies remain under-developed for non-expert users, posing issues for non-expert adoption/use of the technology.

% % Conflicting nature here: It's gonna be the future and change everything yet it's not well understood nor how to make generative AI relevant in entreprenurial contexts, and how 

% % Prior shows how local entrepreneurs leverage their local networks in technology adoption, what do these networks look like and how do they facilitate use of generative AI. How can technology be designed to support social use of generative AI?



% % % What's the simplest way to introduce this? (!)

% % % get to here
% % Generative AI


% % Prior work has shown how technical capacity building 


% % Further, the constant up-skilling required of entreprenuers to stay economically relevant disproportionately effects those in under-resourced contexts. Thus, researchers have explored the various ways in which entreprneuers prefer to engage digital. Prior work studying local entreprenuers 




% % It has been behind X, Y, Z great things for society.

% % Despite this 


% % % and generative AI

% % % but 

% % Despite being praised as a "democratizing force", scholars have pointed out challenges for under-resourced entrepreneurs in constantly ups killing to keep up with the pace of technology to stay relevant, worsening the digital divide. 


% % local entreprenuers, although not definitionally under-resourced by nature of aiming to serve their local economy 

% % Prior scholarship in Human-Computer Interaction (HCI) has investigated different ways in which local entrepreneurs from lean economies engage to keep up with these burdens. \textit{Dillahunt et al}
% % \textit{Hui et al} \textit{Kotturi et al}

% % Be it through peer, expert-connecting organizations, tech-capacity building initiatives

% % In efforts to keep up and acquire necessary tech-skills, local entrepreneurs - who aim to serve their local economy - establish and rely on their local networks. 

% % Recently, advancements in generative AI technology have increased the risks of not upskilling. Increasing the digital divide.
% % Some work has shown how general purpose technology increases entrepreneurial productivity.
% % There are already divides in the adoption and use of generative AI along socio-econonmic, generational, and educational lines.

% % Increasing the risk of not keeping up with the digital divide.

% % Prior work has shown how current interaction paradigms for generative AI is difficult for non-experts. Various approaches have been taken to make the accessibility of interaction paradigms better.


% % Though causal effects on firm use of generative AI technology for business tasks remain unclear 


% % Small local networks are important when acquiring tech skills for local entreprenuers. What do these small networks look like, and how do they facilitate (and/or impede) the use of generative AI?

% % Further, how can technology be designed to support social use of generative AI among local entreprenuers?




% % \section{Introduction | hammer -> nail }
% % The rapid advancement and popularization of generative AI technologies have sparked significant discussions about their transformative potential in the workplace \cite{mckinsey-report}. Despite this potential, there is a growing concern about the widening generational, educational, and socio-economic divides in the use and adoption of these technologies \cite{pewresearch, Koetsier2023, ForbesTechCouncil2023}. Local entrepreneurs, particularly those from resource-limited backgrounds who often engage in entrepreneurship out of necessity \cite{10.1145/3173574.3173814}, stand to benefit from generative AI in automating and enhancing business tasks. However, they also face significant challenges in adopting these advanced technologies due to existing disparities \cite{10.1145/3173574.3173814}.

% % In the field of HCI, research has highlighted the complexities involved in interacting with generative AI systems, especially for non-experts \cite{10.1145/3544548.3581388}. The nuances of prompting and other interaction techniques are not as straightforward as they seem, posing barriers to effective utilization \cite{10.1145/3544548.3581388}. Moreover, the role of peer support and social networks in technology adoption is particularly significant in under-resourced communities \cite{doi:10.1111/etap.12053, GALLOWAY2021101929, 10.1145/3449089}. These insights underscore the need for more accessible and community-oriented approaches to technology implementation, especially in the context of local entrepreneurship \cite{10.1145/3313831.3376363}, \cite{10.1145/3173574.3173814}.

% % However, there remains a gap in understanding the design of generative AI systems for local entrepreneurs, considering their specific challenges and the importance of integrating these technologies within existing social support structures \cite{10.1145/3491102.3501949, 10.1145/3313831.3376363, 10.1145/3491102.3517708} and in the context of onboarding to the technology \cite{kotturi2024deconstructing}. Our study addresses this gap by examining the role of generative AI in the context of local entrepreneurship, particularly focusing on the dynamics of social support and operational challenges.

% % This paper presents findings from a series of speed-dating \cite{ZIMMERMAN201730} interviews conducted with local entrepreneurs and support providers in the Pittsburgh area. Our research is guided by the following questions:

% % \begin{enumerate}
% % \item How should online support systems be built to support entrepreneurs using generative AI?
% % \item How should systems, considering operational challenges associated with current interaction techniques, be designed to support generative AI use with local entrepreneurs?
% % \end{enumerate}

% % We make the following contributions: 
% % \begin{enumerate}

% %     \item outline "danger zones" and design ideas that could be harmful in resource-constrained entrepreneurship.
% % \end{enumerate}



% % ========================
% % \section{Introduction}
% % Studies clearly show the benefits of soliciting peer feedback on entrepreneurial success. 


% Despite this potential, there is a growing concern about the widening generational, educational, and socio-economic divides in the use and adoption of these technologies \cite{pewresearch, Koetsier2023, ForbesTechCouncil2023}.




% are positioned at a crossroads 
% On the one hand, local entrepreneurs are ready to leverage this nascent technology to keep pace with the myriad and varied tasks while required of small business ownership~\cite{Otis2023UnevenImpact}.
% On the other hand, t

% further exacerbating the digital divide \cite{}.


%Such concerns are heightened as local entrepreneurs often operate in under-resourced contexts and lack the infrastructural support to keep up with the constant self-upgrading and technical maintenance required to keep pace in the digital age (i.e., the ``additional labors'' of the digital entrepreneurship~\cite{avle2019additional}) \cite{10.1145/3359320, 10.1145/3274340}.



% Prior work in human-computer interaction (HCI) highlights the benefits of small, local networks for local entrepreneurs in overcoming challenges with technology \cite{10.1145/3491102.3501949, 10.1145/3313831.3376363, 10.1145/3491102.3517708}.
% \yasmine{In this setting, the value of small local networks provides is: A, B, and C}.
% Recent work in HCI investigated the role of social support when introducing local entrepreneurs to generative AI technologies and found that communal exposure to generative AI assuaged the ``techno-anxieties'' associated with such nascent yet powerful technology~\cite{genAIworkshops}.
%Therefore, building on prior scholarship that details how local entrepreneurs leverage their local network when acquiring new technology skills \cite{10.1145/3313831.3376363, 10.1145/3491102.3501949, 10.1145/3359320}, 
% \yasmine{Small local networks are important when acquiring tech skills for local entrepreneurs, therefore we ask:}


%%% Yasmine's doodles 


%% For small-scale entrepreneurs, the non-stop need to keep pace with tech advancements can make or break a business + trusted networks play a pivotal role in this technological maintenance.
%% This is especially the case for entrepreneurs from lean economies, where trusted networks ease the burden of tech maintanence through shared resources, vetted, all within a shared geographic context. 
%% In this paper, we explore the role that trusted networks may play in supporting (and/or disuading or navigating)  entrepreneurs' use of generative AI, where the rapid pace, uncertainty, ... makes use and maintenance esp challenging.
%% Through an exploratory interview study with 7 entrepreneurs and 4 entrepreneur mentors, we probe participants about their current and/or desired experiences leveraging trusted networks when applying gen AI to their business and workflows.
%% For instance, we find that the social use com
%% In doing so, we contribute an initial look at how interventions may be helpful to strengthen entreprenuers' networks around generative AI, for instance by....
%% something about sociotechnical gap?

%% RQ: What does the social context of use around generative AI look like for small-scale entrepreneurs?
%%% RQ: What are the challenges and opportunities for facilitating entrepreneurs' social support networks around using generative AI?





%% Gen AI holds great potential for entrepreneurs, esp those from lean economies
%% Yet, recent work shows how the use of generative AI make the rich get richer, successful entrepreneurs are able to ask good questions, unsuccessful entrepreneurs ask bad questions, get bad results
%% Such a finding follows technological aplification theory, most genAI users have technical background, or are college educated
%% Recent work showcases the importance of local support networks when onboarding entrepreneurs from lean economies to new technologies, for instance, through both offline and online peer and mentor networks.
%% However it is unclear how support networks should be designed in the novel context of generative AI, where the rapid pace of technological advancements..




% Therefore, [one sentence about why this focus of this study matters, as it relates to local entrepreneurship].
% Therefore, while prior work highlights the role of social support when on-boarding local entrepreneurs to generative AI technologies \cite{genAIworkshops}, this work expands upon this by considering the role of entrepreneurs' local networks in critical use of the technology, after on-boarding.
% \yasmine{This role took a few shapes: A, B, and C (make C shared use so that it flows into next sentence)}
% This role took a few shapes: an in-person supportive presence to help build entrepreneurs self-efficacy, online collaborators on prompts, and a wrap-around facilitator to using generative AI technology.



% and but therefore

% more definitional work --> what are these terms?

% Entrepreneurship in the digital age has largely been hailed as a driver for innovation, economic mobility, and social change \cite{10.7551/mitpress/2333.001.0001}. 
% % \yasmine{[one sentence - what is digital entrepreneurship?]}
% Digital entrepreneurship, which is characterized by the use of various electronic means to engage in business \cite{digital-entrepreneurship}, has become a prevalent feature of other types of 21st-century entrepreneurship through the rise of social, e-commerce, and mobile platforms.
% Yet, scholars have questioned the perception of digital entrepreneurship as a ``democracatizing'' force \cite{10.7551/mitpress/2333.001.0001}, surfacing how the constant self-upgrading and technical maintenance required for entrepreneurs to stay relevant disproportionately disadvantages under-resourced and non-technical entrepreneurs \cite{10.1145/3359320, 10.1145/3274340} -- worsening existing digital divides \cite{bbc-digital-literacy, 10.1145/2858036.2858343}. 
% % \yasmine{local entrepreneurship? define and tie in}
% Local entrepreneurs, often focused on small-scale operations in their local economy \cite{10.1145/3313831.3376363}, are especially vulnerable to these digital divides due to the economic limitations arising from their geographic scope.




\section{Introduction}
% probably should cite Ackerman ? socio-technical gap
Generative AI has demonstrated its potential to have a transformative impact on the workplace \cite{mckinsey-report, eloundou2023gpts}. 



by increasing efficiency \cite{Peng2023ImpactOfAIDeveloper}, augmenting creativity \cite{Doshi2023GenerativeAI}, and improving worker output  \cite{Girotra2023IdeasAD}. 
Entrepreneurs who can effectively leverage generative AI for their business, ... have x, y, z benefits

In fact, recent work shows highlights the uneven impact generative AI will have on entrepreneurial performance

Local entrepreneurs, who primarily target their local economy \cite{}, 

In particular, entrepreneurs....
local entrepreneurs...
digital divide...
recent work in hci shows the important of social support (chi '24?)

generative AI potential to exacerbate existing divides \cite{Otis2023UnevenImpact}

At the same, legal uncertainties surrounding intellectual property \cite{mitsloan-generative-ai}, factual inaccuracies in generated content \cite{10.1162/tacl_a_00324}, and new interaction paradigms for generative models \cite{morris2023design} further complicate adopting generative AI into business practices. 

Prior scholarship shows how local entrepreneurs, who aim to serve their local economy, leverage their local network when acquiring new tech-skills \cite{10.1145/3313831.3376363, 10.1145/3491102.3501949, 10.1145/3359320}. 
However, given the myriad of ethical \cite{10.1145/3544549.3585657} and technical challenges \cite{10.1145/3544548.3581388} pertinent to entrepreneurial adoption of generative AI, it is unclear how local entrepreneurs utilize these networks in the context of generative AI. This paper aims to shed light on this area.
% ---------

Therefore, we conducted a Speed Dating \cite{ZIMMERMAN201730} study with  local entrepreneurs and support providers, guided by two main research questions:

% \yasmine{Small local networks are important when acquiring tech skills for local entrepreneurs, therefore we ask:}

\begin{itemize}
    \item \textbf{RQ1}: How do small local networks facilitate, sustain, and impede local entrepreneurs' use of generative AI technologies?
\end{itemize}

Given that generative AI technologies are largely designed for individual use, yet local entrepreneurs benefit from social support when using technology, we ask:

\begin{itemize}
    \item \textbf{RQ2}: How can technology be designed to support social use of generative AI technologies?
\end{itemize}

% Our analysis revealed that entrepreneurs form small local networks for shared use of generative AI through shared accounts, encompassing trusted individuals such as family members, business partners, and peers from in-person incubators. 
Our analysis revealed that entrepreneurs, through trusted peers, incubators, and small business workshops, relied on their small local networks for their introduction and continued use of generative AI technologies.
Despite the single user design of these tools, entrepreneurs appropriated existing systems for shared use (e.g. sharing accounts) to overcome operational barriers, like prompting, to using generative AI and build self-efficacy.
% These networks serve as sources of discovery, showcasing the diverse applications of generative AI, and as mediators, helping to refine requests and ensure practical outputs. 
We observe that sharing use of the technology was critical to keep up with the pace of innovation: entrepreneurs who had the richer, continuous support that shared use affords tended to have more sustained use of generative AI beyond introductions.
Additionally, we observe that local entrepreneurs establish boundaries in their adoption of generative AI, delineating ethical, and sometimes socially construed, boundaries of use, like that between art and business centered tasks. 
Last, we provide initial implications for designing tools supporting social uses of generative AI among entrepreneurs, highlighting the importance of meeting entrepreneurs where they are at through familiar platforms, the dangers of model-centric solutions to providing support, and simple affordances that go beyond chat interfaces to overcome challenges with prompting.

Overall, this research contributes rich empirical data provide an understanding of how local entrepreneurs navigate the burgeoning field of generative AI through an exploratory Speed Dating study with seven local entrepreneurs and four technical providers in the [Removed for Anonymity] area. 
% Specifically, this paper highlights the significance of local networks in not only adopting new technologies but also in shaping their usage in a way that respects their social, ethical, and practical boundaries.
% \yasmine{methodological details?}
Ultimately, these insights pave the way for future work aimed at designing generative AI tools that are more attuned to the complex socio-technical milieu surrounding entrepreneurship.
% ==========================================














% ============= V2 =============
% \section{Introduction}
% Entrepreneurship in the digital age has largely been hailed as force for innovation, economic mobility, and social change \cite{10.1145/3274340}. However, scholars have brought these notions into question, surfacing how the constant self-upgrading and technical maintenance required for entrepreneurs to stay relevant disproportionately disadvantages under-resourced and non-technical entrepreneurs \cite{10.1145/3359320} --- worsening existing digital divides \cite{bbc-digital-literacy}. Prior scholarship has made light on how entrepreneurs leverage peer networks for 


% Prior scholarship highlights entrepreneurs engage peers to meet the demands of digital age \cite{}. From feedback seeking on social media to blah blah for blah blah. 

% Recently, generative AI technologies have garnered attention for their transformative impact on the workplace \cite{mckinsey-report, eloundou2023gpts}, demonstrating increased efficiency, augmented creativity, and improved worker output associated with it's use \cite{Doshi2023GenerativeAI, Girotra2023IdeasAD, Peng2023ImpactOfAIDeveloper}. Though the causal effects of generative AI on entrepreneurial performance remain unclear \cite{Otis2023UnevenImpact}, the hype-driven rhetoric surrounding the technology and it's initial promise create a uniquely high pressure to adapt or be left behind. At the same, legal uncertainties surrounding intellectual property \cite{mitsloan-generative-ai}, factual inaccuracies in generated content \cite{10.1162/tacl_a_00324}, and new interaction paradigms for generative models \cite{morris2023design} further complicate adopting generative AI into business practices. Given the myriad of ethical and technical challenges pertinent to entrepreneurial adoption of generative AI, it is unclear how local entrepreneurs utilize these networks in the context of generative AI. This paper aims to shed light on this area.
% % ---------

% Therefore, we conducted a Speed Dating \cite{ZIMMERMAN201730} study with  local entrepreneurs and support providers, guided by two main research questions: \textbf{RQ1}: Small local networks are important when acquiring tech skills for local entrepreneurs, what do these small local networks look like, and how do they facilitate and/or impede use of generative AI technologies? \textbf{RQ2}: How can technology be designed to support social use of generative AI technologies?

% Our analysis revealed that entrepreneurs form small local networks for shared use of generative AI through shared accounts, encompassing trusted individuals such as family members, business partners, and peers from in-person incubators. Despite the individual-centric design of these tools, the communal approach to their use is critical to keeping up with the pace of innovation. These networks serve as sources of discovery, showcasing the diverse applications of generative AI, and as mediators, helping to refine requests and ensure practical outputs. Additionally, we observe that local entrepreneurs establish boundaries in their adoption of generative AI, delineating social, ethical, and practical parameters to guide its use. Last, we provide initial implications for designing tools supporting social uses of generative AI among entrepreneurs.

% Overall, this research contributes to a deeper understanding of how local entrepreneurs navigate the burgeoning field of generative AI. It highlights the significance of local networks in not only adopting new technologies but also in shaping their usage in a way that respects social, ethical, and practical boundaries. Ultimately, these insights pave the way for future work aimed at designing generative AI tools that are effective and attuned to the varied landscapes of entrepreneurial innovation.

% maybe i need something justifying the second question more; like current technologies don't surround the use of social support;
%       - gen AI is a collaborator
%       -  while entreprenuers engage in peer-feedback for other things in the ideation process 
%  generative AI as a collaborator in certain entreprenuership processes;
% the current design of generative AI technologies doesn't revolve around these collaborative processes
% there is a framework for this -- i just forget the paper (but the creative writing x generative AI paper, does look at it)








% Prior scholarship in human-computer interaction (HCI) investigates various ways in which local entrepreneurs from lean economies 
% % here, kotturi, dillahunt, hui;

% While these models for social support 

% Prior work shows the role of peer support in ---, ---, and ----. This authors shows how entrpeenures utilize feedback for -----. While --- expands on this by showing how entreprenurs ----. Alas,



% Prior scholarship has shown how local entrepreneurs - who aim to serve their local economy - rely on their local networks in


% From Otis et al 2023:
% Consistent with the optimism currently surrounding generative AI (AI hereafter), recent experiments show that conversing with and receiving AI assistance causes workers to write faster  and  better  business  text,  including  press  releases,  ad  copy,  consulting  memos,  and customer support messages (Brynjolfsson, Li, and Raymond, 2023; Dell’Acqua et al., 2023;Doshi and Hauser, 2023; Noy and Zhang, 2023; Chen and Chan, 2023).



% Prior scholarship studying how local entrepreneurs - who aim to serve their local economy - from lean economies leverage their local networks when acquiring technical skills by engaging community resources, peers, and tech capacity building programs \cite{}. However, it remains unclear how local entrepreneurs leverage these networks in navigating the landscape of generative AI. In this study we ask the following questions:

% Yet, how entrepreneurs, particularly those from low-tech backgrounds, adopt generative AI technologies remains unclear. Further, HCI researchers have highlighted how current interaction paradigms for generative AI (e.g. prompting) are not conducive to non-expert users.
% I don't like this sentence.
% \begin{enumerate}
%     \item Small local networks are important when acquiring tech skills for local entrepreneurs, what do these small local networks look like, and how do they facilitate and/or impede use of generative AI technologies?
%     \item Further, how can technology be designed to support social use of generative AI technologies?
% \end{enumerate}

% In this paper we present the empirical findings from a Speed Dating \cite{ZIMMERMAN201730} study with seven local entrepreneurs and four providers of entrepreneurship support in the greater [CITY] area. We find that even though use is designed for the individual, entrepreneurs assemble small local networks to use generative AI through shared accounts, entrepreneurs establish social, ethical, and economic boundaries of use. Further we present initial implications for designing technology to support entrepreneurs in using generative AI. 







% Technical Barriers with up-keep.
% Prior work studying how local entreprneurs overcome these technical barriers relying on their local networks through peers, community, tech-capacity building.

% Recently, Discussion around generative AI and its impact on workplace performance. Studies showing increased efficiency with generative AI in the firm. Despite this, entreprenuers leveraging generative AI have to deal with a range of complexity unseen with other technologies, such as ethical issues with ownership, IP, humanity (with art? what does art mean, what does it mean to be human?) hallucinations, fast-pace and hype driven rhetoric, At the same time HCI research has shown how the interaction paradigms for generative AI technologies remain under-developed for non-expert users, posing issues for non-expert adoption/use of the technology.

% Conflicting nature here: It's gonna be the future and change everything yet it's not well understood nor how to make generative AI relevant in entreprenurial contexts, and how 

% Prior shows how local entrepreneurs leverage their local networks in technology adoption, what do these networks look like and how do they facilitate use of generative AI. How can technology be designed to support social use of generative AI?



% % What's the simplest way to introduce this? (!)

% % get to here
% Generative AI


% Prior work has shown how technical capacity building 


% Further, the constant up-skilling required of entreprenuers to stay economically relevant disproportionately effects those in under-resourced contexts. Thus, researchers have explored the various ways in which entreprneuers prefer to engage digital. Prior work studying local entreprenuers 




% It has been behind X, Y, Z great things for society.

% Despite this 


% % and generative AI

% % but 

% Despite being praised as a "democratizing force", scholars have pointed out challenges for under-resourced entrepreneurs in constantly ups killing to keep up with the pace of technology to stay relevant, worsening the digital divide. 


% local entreprenuers, although not definitionally under-resourced by nature of aiming to serve their local economy 

% Prior scholarship in Human-Computer Interaction (HCI) has investigated different ways in which local entrepreneurs from lean economies engage to keep up with these burdens. \textit{Dillahunt et al}
% \textit{Hui et al} \textit{Kotturi et al}

% Be it through peer, expert-connecting organizations, tech-capacity building initiatives

% In efforts to keep up and acquire necessary tech-skills, local entrepreneurs - who aim to serve their local economy - establish and rely on their local networks. 

% Recently, advancements in generative AI technology have increased the risks of not upskilling. Increasing the digital divide.
% Some work has shown how general purpose technology increases entrepreneurial productivity.
% There are already divides in the adoption and use of generative AI along socio-econonmic, generational, and educational lines.

% Increasing the risk of not keeping up with the digital divide.

% Prior work has shown how current interaction paradigms for generative AI is difficult for non-experts. Various approaches have been taken to make the accessibility of interaction paradigms better.


% Though causal effects on firm use of generative AI technology for business tasks remain unclear 


% Small local networks are important when acquiring tech skills for local entreprenuers. What do these small networks look like, and how do they facilitate (and/or impede) the use of generative AI?

% Further, how can technology be designed to support social use of generative AI among local entreprenuers?




% \section{Introduction | hammer -> nail }
% The rapid advancement and popularization of generative AI technologies have sparked significant discussions about their transformative potential in the workplace \cite{mckinsey-report}. Despite this potential, there is a growing concern about the widening generational, educational, and socio-economic divides in the use and adoption of these technologies \cite{pewresearch, Koetsier2023, ForbesTechCouncil2023}. Local entrepreneurs, particularly those from resource-limited backgrounds who often engage in entrepreneurship out of necessity \cite{10.1145/3173574.3173814}, stand to benefit from generative AI in automating and enhancing business tasks. However, they also face significant challenges in adopting these advanced technologies due to existing disparities \cite{10.1145/3173574.3173814}.

% In the field of HCI, research has highlighted the complexities involved in interacting with generative AI systems, especially for non-experts \cite{10.1145/3544548.3581388}. The nuances of prompting and other interaction techniques are not as straightforward as they seem, posing barriers to effective utilization \cite{10.1145/3544548.3581388}. Moreover, the role of peer support and social networks in technology adoption is particularly significant in under-resourced communities \cite{doi:10.1111/etap.12053, GALLOWAY2021101929, 10.1145/3449089}. These insights underscore the need for more accessible and community-oriented approaches to technology implementation, especially in the context of local entrepreneurship \cite{10.1145/3313831.3376363}, \cite{10.1145/3173574.3173814}.

% However, there remains a gap in understanding the design of generative AI systems for local entrepreneurs, considering their specific challenges and the importance of integrating these technologies within existing social support structures \cite{10.1145/3491102.3501949, 10.1145/3313831.3376363, 10.1145/3491102.3517708} and in the context of onboarding to the technology \cite{kotturi2024deconstructing}. Our study addresses this gap by examining the role of generative AI in the context of local entrepreneurship, particularly focusing on the dynamics of social support and operational challenges.

% This paper presents findings from a series of speed-dating \cite{ZIMMERMAN201730} interviews conducted with local entrepreneurs and support providers in the Pittsburgh area. Our research is guided by the following questions:

% \begin{enumerate}
% \item How should online support systems be built to support entrepreneurs using generative AI?
% \item How should systems, considering operational challenges associated with current interaction techniques, be designed to support generative AI use with local entrepreneurs?
% \end{enumerate}

% We make the following contributions: 
% \begin{enumerate}

%     \item outline "danger zones" and design ideas that could be harmful in resource-constrained entrepreneurship.
% \end{enumerate}



% ========================
% \section{Introduction}
% Studies clearly show the benefits of soliciting peer feedback on entrepreneurial success. 

==> Paper_Content/3_storyboard-table.tex <==
\begin{table}[H]
\centering
\begin{tabular}{c}
\begin{minipage}{0.4\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Appendix Content/storyboard_25.jpeg}
\end{minipage}
\\
\begin{minipage}{0.4\textwidth}
  \centering
  \includegraphics[width=\textwidth]{Appendix Content/storyboard_26.jpeg}
  \captionof{figure}{Storyboard 26}
  \label{fig:appendixImage2}
\end{minipage}
\end{tabular}
\caption{Storyboards 25 and 26}
\label{fig:storyboards}
\end{table}


% \documentclass{article}
% \usepackage[table]{xcolor}
% \usepackage{multirow}
% \usepackage{makecell}
% \usepackage{hhline}
% \usepackage{array}
% \usepackage[letterpaper, left=0.5in]{geometry}



% % set special column width for storyboard color cells
% \newcolumntype{C}{>{\centering\arraybackslash}p{0.02cm}}

% % set row height, globally
% \newcommand{\fixedheightcell}[2][1.5cm]{\begin{tabular}[b]{@{}c@{}}\rule{0pt}{#1}#2\end{tabular}}

% \definecolor{local}{RGB}{191, 225, 246} % Red
% \definecolor{community}{RGB}{255, 229, 160} % Green
% \definecolor{peer}{RGB}{212, 237, 188} % Blue
% \definecolor{multiple}{RGB}{230, 207, 242} % Multiple
% \definecolor{other}{RGB}{255, 207, 201}

% % What? (colors)
% \definecolor{SMS}{RGB}{255,207,201}
% \definecolor{groupchat}{RGB}{198,219,225}
% \definecolor{Browser}{RGB}{117,56,0}
% \definecolor{Email}{RGB}{33,90,108}
% \definecolor{Learning Module}{RGB}{71,56,34}
% \definecolor{video}{RGB}{33,90,108}
% \definecolor{custom model}{RGB}{61,61,61}
% \definecolor{spreadsheet}{RGB}{10,83,168}

% % When? (colors)
% \definecolor{Before}{RGB}{130,174,241}
% \definecolor{During}{RGB}{255,0,219}
% \definecolor{After}{RGB}{255,137,0}
% \definecolor{Multiple Stages}{RGB}{255,235,0}
% \definecolor{N/A}{RGB}{59,255,0}

% % How? (colors)
% \definecolor{AIH}{RGB}{10, 83, 168}
% \definecolor{AI}{RGB}{230, 207, 242}
% \definecolor{Human}{RGB}{255, 200, 170}
% \definecolor{Neither}{RGB}{17, 115, 75}



% \begin{document}

    


% \begin{table}[t]
% \renewcommand{\arraystretch}{0.5}
% \begin{tabular}{|p{7.5cm}|*{27}{C|}} 
% \hline
% \rowcolor{gray!10}
% \hline
% Storyboard \# & 1 & 2* & 3* & 4* & 5* & 6 & 7 & 8* & 9* & 10* & 11 & 12 & 13* & 14* & 15* & 16 & 17* & 18* & 19* & 20* & 21* & 22 & 23 & 24* & 25* & 26* \\ 

% \hline

% % Who? (colors)

% \begin{tabular}{ll}
%  \textbf{Who?} & 
%  \begin{tabular}{ll}
%     \small Local Provider \textcolor{local}{\rule{2mm}{2mm}} & 
%     \small Multiple \textcolor{multiple}{\rule{2mm}{2mm}} \\
%     \small Community Provider \textcolor{community}{\rule{2mm}{2mm}} &
%     \small Peer \textcolor{peer}{\rule{2mm}{2mm}} \\
%  \end{tabular}
% \end{tabular}

%  & \cellcolor{multiple} & \cellcolor{multiple} & \cellcolor{community} & \cellcolor{community} & \cellcolor{community} & \cellcolor{local} & \cellcolor{peer} & \cellcolor{peer} & \cellcolor{multiple} & \cellcolor{multiple} & \cellcolor{local} & \cellcolor{local} & \cellcolor{community} & \cellcolor{peer} & \cellcolor{peer} & \cellcolor{community} & \cellcolor{multiple} & \cellcolor{local} & \cellcolor{local} & \cellcolor{community} & \cellcolor{peer} & \cellcolor{other} & \cellcolor{other} & \cellcolor{community} & \cellcolor{peer} & \cellcolor{community} \\
 
% \hline

% \begin{tabular}{ll}
%  \textbf{What?} & 
%  \begin{tabular}{ll}
%     \small SMS \textcolor{SMS}{\rule{2mm}{2mm}} & 
%     \small Group Chat \textcolor{groupchat}{\rule{2mm}{2mm}} \\
%     \small Browser \textcolor{Browser}{\rule{2mm}{2mm}} & 
%     \small Email \textcolor{Email}{\rule{2mm}{2mm}} \\
%     \small Learning Module \textcolor{Learning Module}{\rule{2mm}{2mm}} & 
%     \small Video \textcolor{video}{\rule{2mm}{2mm}} \\
%     \small Custom Model \textcolor{custom model}{\rule{2mm}{2mm}} & 
%     \small Spreadsheet \textcolor{spreadsheet}{\rule{2mm}{2mm}} \\
%  \end{tabular}
% \end{tabular}

%  & \cellcolor{groupchat} & \cellcolor{groupchat} & \cellcolor{SMS} & \cellcolor{custom model} & \cellcolor{custom model} & \cellcolor{custom model} & \cellcolor{Email} & \cellcolor{Browser} & \cellcolor{groupchat} & \cellcolor{Learning Module} & \cellcolor{Learning Module} & \cellcolor{Browser} & \cellcolor{other} & \cellcolor{groupchat} &\cellcolor{Browser} & \cellcolor{spreadsheet} & \cellcolor{SMS} & \cellcolor{custom model} & \cellcolor{custom model} & \cellcolor{Browser} & \cellcolor{groupchat} & \cellcolor{other} & \cellcolor{other} & \cellcolor{SMS} & \cellcolor{other} & \cellcolor{video} \\

% \hline

% \begin{tabular}{ll}
%  \textbf{When?} & 
%  \begin{tabular}{ll}
%     \small Before \textcolor{Before}{\rule{2mm}{2mm}} & 
%     \small During \textcolor{During}{\rule{2mm}{2mm}} \\
%     \small After \textcolor{After}{\rule{2mm}{2mm}} & 
%     \small Multiple Stages \textcolor{Multiple Stages}{\rule{2mm}{2mm}} \\
%     \multicolumn{2}{l}{\small N/A \textcolor{N/A}{\rule{2mm}{2mm}}} % Spanning entire row
%  \end{tabular}
% \end{tabular}
%  & \cellcolor{During} & \cellcolor{During} & \cellcolor{Before} & \cellcolor{During} & \cellcolor{During} & \cellcolor{Before} & \cellcolor{Before} & \cellcolor{During} & \cellcolor{During} & \cellcolor{During} & \cellcolor{During} & \cellcolor{During} & \cellcolor{During} & \cellcolor{Before} & \cellcolor{During} & \cellcolor{After} & \cellcolor{Before} & \cellcolor{After} & \cellcolor{After} & \cellcolor{After} & \cellcolor{During} & \cellcolor{Multiple Stages} & \cellcolor{After} & \cellcolor{N/A} & \cellcolor{Before} & \cellcolor{Before} \\

% \hline

% \begin{tabular}{ll}
%  \textbf{How?} & 
%  \begin{tabular}{ll}
%     \small AI+Human \textcolor{AIH}{\rule{2mm}{2mm}} & 
%     \small AI only \textcolor{AI}{\rule{2mm}{2mm}} \\
%     \small Human only \textcolor{Human}{\rule{2mm}{2mm}} & 
%     \small Neither \textcolor{Neither}{\rule{2mm}{2mm}} \\
%  \end{tabular}
% \end{tabular}
%  & \cellcolor{AIH} & \cellcolor{AIH} & \cellcolor{AIH} & \cellcolor{AI} & \cellcolor{AI} & \cellcolor{AIH} & \cellcolor{Human} & \cellcolor{AIH} & \cellcolor{AIH} & \cellcolor{AIH} & \cellcolor{AIH} & \cellcolor{Human} & \cellcolor{Neither} & \cellcolor{Human} & \cellcolor{Human} & \cellcolor{Human} & \cellcolor{Human} & \cellcolor{AIH} & \cellcolor{AIH} & \cellcolor{AI} & \cellcolor{AIH} & \cellcolor{AI} & \cellcolor{AI} & \cellcolor{Human} & \cellcolor{Human} & \cellcolor{Human} \\

% \hline

%  % Why? (colors)
% % \definecolor{}{RGB}{,,,}


% % \yasmine{There needs to be a description somewhere of buckets of scenarios of the storyboards as they respond to major pain points for local entrepreneurs, such as 1. organizing business tasks, 2. generating content (for social media, websites, etc), 3. ... etc. If the why/what/how/when structure makes sense above, maybe this missing link can be phrased as the ``why''}

% \begin{tabular}{ll}
%  \textbf{Why?} & 
%  \begin{tabular}{ll}
%     \small Placeholder \textcolor{local}{\rule{2mm}{2mm}} & 
%  \end{tabular}
% \end{tabular} & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 \\

% \hline

% \end{tabular}
% \caption{Storyboards were generated to represent a large range of the design space}

% \end{table}

% \end{document}

==> Paper_Content/4_Findings-OLD.tex <==
% Remember: Your Results section speaks for itself: report on the results of your work in an organized way. Refrain from reporting on the significance of these results until the Discussion section, which comes next. 

% "For now, report on the results dispassionately. Use charts, graphs, and tables as appropriate. Good Results sections do not simply jam a bunch of numbers in, but “tell a story with data,” creating an easy-to-read narrative flow that does not make the reader do too much work to figure out what happened."
% ===================================
\section{Findings}
% boundaries of use
% which storyboards bring up these reflections
% quotes around the storyboards
% in response 
% tying to storyboard helps to make the claim more focused ... not 
% narrow the scope, play safer by referencing storyboards...


% ========================================
\subsection{Social Underpinnings of Generative AI}

% Do you think 'trusted' needs to be justified more throughout here?
\subsubsection{Shared Use}
Despite mainstream generative AI technologies being designed for individual use, entrepreneurs assemble small local networks to use generative AI systems though shared accounts, which comprise trusted individuals such as family members, business partners, and peers met through in-person incubators (E1, E2, E5, E6).
% this characterization of "shared use" semes rather vague --> what comprises shared use. The extent and form of shared use is rather different. What comprises "shared accounts" --> also has the potential to be vague.
Sharing use of generative AI technologies was motivated by three factors: X, Y, and Z. 
First, consistent with literature highlighting entrepreneurial resourcefulness in lean economies \cite{}, entrepreneurs shared accounts to save costs.
LE1, shared a ChatGPT account with his business partners with which they rotate who pays each month. Similarly, E5 acknowledged that she could use her own ChatGPT account, but it made more sense to use her husband's considering he paid for the Premium model.
While the motivation to share accounts (for entrepreneurs who were) was initially cost-saving, entrepreneurs reflected on the emergent benefits of their shared use. 
While E5 shared an account with her husband, the nature of her interaction with generative AI changed from prompting a system, to having a conversation about her needs, followed by him facilitating the prompting process.
E1 highlighted how by seeing other's prompts he can learn more quickly from other's trials and errors, \textit{"I don't have to try and fail a lot of times. ...I only have to [fail] once or twice because I've seen six other people try and fail in different ways."}
% Beyond the passive learning off of other's prompts LE1 would FaceTime teammates to share, fail, and ultimately learn, synchronously.
\yasmine{insert quote interpretation - what does failure mean here?}
For E2, shared, in-person use with technical provider at a community center helped her build the self-efficacy to get started, [describe more about the format of this set up, something like: In particular, E2 referenced a recent community workshop she attended which partnered an entrepreneur with a technical expert for side-by-side support.....or something. From this experience, E2 reflected:``When we were able to sit around the table and you got to sit with a [provider] ... [That] makes you feel like you can do it yourself and it makes you feel at ease.`` 
\yasmine{quote interpretation, what is important to attend to in this quote?}
For entrepreneurs and providers not implicated in shared use, they reflected on the potential benefits that other entrepreneurs realized. 
For instance, E3 shared how she could see herself, ''developing my own skillset by emulating or using other folks as a starting point'' by sharing an interface where you could see other entrepreneurs prompts.
P1 and P2 suggested how in pairing up interested entrepreneurs, who had a shared context (e.g. community center), to share an interface could "bridge the gap [of] comfort around these tools" (P2). 
% don't like this sentence --> trying to bridge 
While the local networks that entrepreneurs formed around the use of generative AI did not always lead to shared use, they often facilitated the necessary introductions and assistance to stay technologically relevant in the digital age.
% \yasmine{weren't there things about not wanting shared use? Is that in boundaries of use section? Maybe hint to it here or maybe during the introduction of this subsection- TBD like "in Section~\ref{} we discuss..."}


% === thought kernel  *trust* ====
% LE2 shares that she usually text her husband or a trusted provider, when she's trying to get help using ChatGPT. 
% EP1 says, "I probably wouldn't have gone to ChatGPT if a trusted friend hadn't suggested it." She reflects how the person who introduces her to ChatGPT "can't just be anyone," rather someone who's opinion about technology she respects and trusts. 

% In sharing use, \textit{trust} was paramount. 
% Maybe more text here to the effect of: 'although not entreprneuers shared, the reaction to systems in which they could collaborate on chat interfaces was well recieved, and many pointed out the benefits that come along with the collaboration' --> or would this be later
% cella talks about how being a supportive presence is really important to her work at tech help;
% The ways in entrepreneurs leveraged shared accounts varied depended on their use case. In a less formal way, LE5 describes using ChatGPT by proxy of her husband. 
% Savion, Bhavya, Jarmele, shared use of the tech
%   - all through shared accounts
%   - Kyrie, keegan "taught me how to use ChatGPT"
% ========================

% needs more about entreprenuers feeling like they will be left behind to start this. 

% =========================
\subsubsection{Keeping Up}
\yasmine{[some kind of intro like With the rapid pace of technological change of genAI...,]} the local entrepreneurs in our study and technical providers consistently express the concern of being "left behind." 
\yasmine{This meant:}
Because of this, entrepreneurs shared our small, local networks were critical to "keep up" with pace of innovation by providing a both a source of discovery (e.g., ...) and mediation (e.g., ...). 
% ======== Discovery ========
Some tech providers proactively took on? the role in the communities that they serve to encourage discovery, \yasmine{this quote needs more introduction, there is no preparation for the comment about digital divide}
\begin{quote}
    “Even if I don’t necessarily feel that I’m on the other side of the divide yet, I certainly encourage the entrepreneurs and the other contractors and freelancers and business folks that I work with ... [to learn about] generative AI” (P4).
\end{quote}
\yasmine{quote interpretation}
E6, who recently participated in an X-month long business incubator with her business partner, shared how another entrepreneur taught her how to use ChatGPT (even though this was not part of the formal curriculum).
As E3 in describing her concerns to a trusted friend was encouraged to take a class on Udemy class on prompting basics.
In facilitating discovery, trust was key. P3 made it clear: "I probably wouldn't have gone to ChatGPT if a trusted friend hadn't suggested it." 
% redundant ? thick descriptions?
She reflects how the person who introduces her to ChatGPT "can't just be anyone," rather someone who's opinion about technology she respects and trusts. 
% ======== Mediation ========
Entrepreneurs who shared use, described how mediation others provide helped to overcome operational barriers to using the technology. 
% (!!!) people have some tether to some business support group. How do you talk about this in a way that doesn't assume any background knowledge. (e.g. LE2, who attends a weekly tech program that provides support for entreprenuers, ...) (!!!)
E2 frequently reaches out to providers she knows or her husband when she has trouble prompting.  
Even further, E5 describes how when chatting with her husband about her business, he will point out a use case for ChatGPT and then create the prompt for her: acting as a translator of her needs and mediator to using the technology. 
However, in the end, while local networks facilitated discovery and mediation, the entrepreneurs who didn't have the wrap-around support that shared use affords ended up turning back to familiar tools like Google Search and old practices.


% Kyrie, introduction through incubator
% addressing the comfort gap; although not all entreprenurs shared use. Most when shown storyboards of socially situated use, shared insights 
% Savion, who shared accounts; shared learning; Alicia tho not implicated in account sharing, notes the benefits of peer-to-peer learning in systems enabling entreprnuers to share use
% 
% Erin, via close friend saw how she could use generative AI through reaching out to a friend when she had a problem. Her friend served as the mediator in this case.
% Left behind:
%   - Bhavya scared of being left behind; Her husband serves as the                 proxy/mediator to her use Translating problem to prompt 
%   - Ariel
%   - meg
% LE2 and LE6 shared how their introduction to ChatGPT was from workshop/incubator


% \subsubsection{Trust} --> or this could be talked about throughout this section
% Erin talks about how it was trusted friend who introduced her and if it wasn't she wouldn't have used
% Jarmele may mention trust?
% need to explore if this can be finding;
% erin also talks about how entreprenuers wouldn't trust AI to do some business tasks, saying 'i can just do it myself'

% I don't like the name "Falling behind", but I'm trying to make the narrative with the data to this section that 
% \subsubsection{Falling Behind}

% While LE6 was taught how to use ChatGPT by a peer at an incubator, she describes using it infrequently in ways where it doesn't "sophisticated thesaurus"


% (!) (!) (!) Highlighting a gap between discovering how to use the technology and then actually using the technology (!) (!) (!)

% Something along the lines of, while the motivation may be there, look they talked about being left behind so much -- they had the discovery network


% While entrepreneurs consistently reflected on being left behind, many didn't move past discovery while generative AI.


% ========================================
\subsection{Boundaries}
While, entrepreneurs' social uses of generative AI were critical in keeping up, X, Y, Z, entrepreneurs and providers shared concerns for use in a social context, and beyond. 
for instance, three key drawbacks for ... included: social pressures and reputational concerns, ..., and ethical concerns. 
\yasmine{Something like: these issues where heightened given the unique constraints of small business ownership or...}
To respond to these issues, entrepreneurs contemplated boundaries for use, that is: \yasmine{define}. Here we share the various boundaries entrepreneurs implemented to safeguard themselves from various uses of generative AI. 

\subsubsection{Social Boundaries in Generative AI}
in heightening questions of self-efficacy and introducing ill-understood standards of behavior shared generative AI spaces.
P2 highlights how shared use of generative AI tools intensified her feelings, and the feelings of the entrepreneurs she works with, of being left behind, especially when there's a gap in proficiency. 
This sentiment was echoed by E4, who would be scared to use a “stupid” prompt when exploring, especially when others might witness. 
Further, entrepreneurs considered what appropriate behavior was in a shared use of generative AI versus a personal use. 
E1 details his decision-making process about when to use a personal account versus a shared one: He will actively choose to use a personal account, despite the worse model, when working on personal projects as to not “clutter” the space or ``make anybody mad.''
E3, who preferred to be an observer to others' use of generative AI, while deferring her exploration to a personal account, questions whether not contributing would be accepted by others.
E2 reflected on how she would be "careful" that who she shares use with has the same "core values" and "work ethics".
\yasmine{E2 wants to be work with people who have a similar work ethic, not too techy b/c....}





% demoralizing nature if not at same level - alicia 
% - “I also think a realistic possibility is that Ash is completely demoralized because Mari is going and getting things so much faster than Ash is and Ash just feels like this is not something that I know how to do.”

% For E4, social stigma around the use of generative AI 
% LE4: concern looking stupid:
% Despite this, she expresses her concern of “looking stupid” among other entrepreneurs and the potential judgment associated with her experimentation (ex/ “What’s that possibly gonna do for her business?”).





%  “I think it can’t just be anyone, ‘cause I don’t really value everyone’s opinions when it comes to technology. I value certain people’s opinions. And so if certain people that I value tell me that ChatGPT could be useful for me, and then they show me how to use it, then I’m more likely to use it.” - Erin EP1



% having the same work ethic as another - jarmele
% "you just have to have to make sure that who you're working with or partnering with has kind of like the same core values that you do." - jarmele



% boundaries! socially implicated boundaries!
% LE4 Haylee: “I was with a group of artists who have a little collective and they were trying to generate a press release for an art  show that they were having, And I, I was like helping them come up with ideas and all of them kind of refer to ChatGPT as something that they use really often, that is just part of the norm for them, which I thought was really interesting  ‘cause it’s not something that I go to a ton.” 

% ========= Trust in socially implicated use? ==========
% infringing on safe spaces - jarmele, cella, alicia
% Entrepreneurs and providers (LE2, EP1, EP2) drew boundaries related to the \textit{spaces} where models should train off of. Responding to futures that trained models to support entrepreneurs based off conversations in community spaces, such as in-person incubators or entrepreneurship hubs,  entrepreneurs and providers emphatically pushed back. Entrepreneurs and providers (LE2, EP1, EP2) discuss how training a model based of conversations in community spaces, undermined would infringe on the trust that in-person social support affords.
% ======================================================


% jarmele - let's not do this in tech help
% alicia - I would not be a provider if they made me do this'
% Savion LE1, and Cella LE2. Left room, suggesting only if the usefulness was high enough would they let the model-based solution come in to build context


\subsubsection{Discovery ?? Practicality}
While the entrepreneurs' in our study felt pressured to adopt generative AI systems into their workflows, local networks helped entrepreneurs cut through the hype and understand when using generative AI made sense.
For example, one provider asks the question "why generative AI" to make sure the tech matches the needs, and help entrepreneurs navigate the complex ethical landscape related to the technology:
\begin{quote}
 Because I do think like coming into [Community Center] as part of [Tech Assistance Program], we want to help and do what people need and want. But also, we should provide our lens of like technical expertise, I think. And that should involve helping people learn [to]... understand [what] is and is not useful to them, what is and is not hypey or problematic or harmful in certain ways." (P1)
\end{quote}
Providers shared how centering practicality is particularly important with local entrepreneurs given constrained resources, so when discovering potentially beneficial new technologies the goal should be centered around a practical outcome "instead of making a doodad."
Bringing this into reflections on system design, providers indicated that gamified solutions clearly breach this balance between discoverability and practicality by providing no immediate value to the entrepreneur, and in some cases replicating the "infantalizing nature" of certain participatory design practices (P1). 

% ======== Nugget of Data =======|
% Erin talks about centering practicality, and how she just uses Google Search over ChatGPT

% Erin compares use to a laser cutter workshop she had where she switched from making a toy to something that fit in the process of business
% As a provider, EP3 compared balancing discovery and practicality to a laser-cutting workshop she held at her incubator. Where originally she made the goal of the workshop making a miniature catapult, she changed 
% She suggests that for entrepreneurs learning to use generative AI, the discovery should still be centered around a practical outcome "instead of making a doodad that's like a cool doodad."
% ================================|

% "how people can learn how to use these machines in order to make money off the things that they're making. Um, instead of just like making a doodad that's like a cool doodad"



% Alicia - suggesting low-tech solutions (like tutorials)
% Cella - lowest tech solution for the present need
%               - "why generative AI"
% Alicia --> gamified solutions; don't make money - why use
% Cella --> gamified solutions; don't make money - why use
% Alicia suggesting, if not centering practicality; there should be something else to it (!), in person component, Alicia suggests ... or a family fun activity (modes of interaction)

% Sasha also just uses Google Search
% Kyrie - if it wasn't for social media, kyrie didn't want it
% here we can introduce that they suggested low-tech solutions, yet
% jarmele on 

% (!) centering making money (!)


\subsubsection{Ethical Boundaries}
% this sentence needs work
Entrepreneurs and providers shared ethical concerns regarding generative AI systems including authenticity, transparency, and representation.
Often these concerns dictated use (or lack of use), and therefore took on the form of ethical boundary setting.
For entrepreneurs using generative AI to simplify business tasks was
\begin{quote}
“I have less moral quandary with using AI for my business than I do my art stuff ‘cause the art stuff feels like a personal reflection of my intellect and the business stuff - It’s like, well, this is a business. … I have to participate in capitalism, so I don’t mind [getting] as much help as I can with that to make  money I need to make a living wage, you know? But when it comes to my own artistic stuff, [there are some] ethical things around it that is hard.” (E4) 
\end{quote}
\yasmine{quote interpretation}
Yet, the line between art and business for entrepreneurs was often unclear and subject to the personal values of the entrepreneur. 
While LE4 would not use ChatGPT for ideation purposes, her business partner, E6 had no problem using it to generate Instagram captions based off of the brand she had built out.
Delineating between art and business often meant entrepreneurs had to reflect upon what it means to be artistic, and how their reflection interacts with their occupational identity. 
E6, who preferred to describe her marketing role in her business as "storytelling" to retain a feeling of authenticity, didn't mind generating captions with ChatGPT, despite being part of her brand's marketing, because she believed generating captions was 
On the other hand, E7 shared that "art is in the idea" and "if you can dream it, you can do it" 
Although she did not generate art for products, she did not take issues with entrepreneurs doing so as long as they were transparent in sharing their use of generative AI.
Transparency was not just implicated in \textit{what} generative AI produced but in \textit{how} it was produced.
Even in automating business tasks with generative AI, P3 shared how many of the entrepreneurs in her incubator, would not trust "some random robot or algorithm" to take over tasks without understanding "what's in the secret sauce" or what data is being fed to the model to train it.
Reflecting on serving entrepreneurs of marginalized gender identities, P3 shared that if she were creating content with generative AI, she would want the model to have an "affirmative action bias" so that it can serve the "clients [she is] trying to serve".
\yasmine{err this quote will need some explanation}
% Not sure how valid statement below is --> b/c the storyboard was presented in the context of a community 
While acknowledging this, P3 and P1, questioned the ethics of training a model that is more attuned to local entrepreneurs needs, citing the power imbalance between the creators of the model and the entrepreneurs the model seeks to serve.
\yasmine{be sure to touch of model-based solutions in your third subsection in the findings}


% Further, both entrepreneurs and providers drew lines with model-based solutions which could exacerbate problems with power 

% Yet, noted how with transparency as to how the generative model is being trained 

% nuance to it


% Meg LE3 -> creative tasks, human touch
% sasha LE7 -> creative tasks, artistry is in the idea;
% kyrie LE6 -> creative tasks, human touch
% flexible approaches for what it means to be human
%       -> sasha: 'art is in the idea'
%       -> kyrie: ~'lean into what cannot be automated away'

% haylee LE4 --> social stigma surrounding using genAI
%       - unsure

% sasha --> unclear how others fear about it
% sasha LE7 -> hestitancy around discussing generative AI around peers because of perception in the workplace
% alicia -> environmental impact of generative AI

% 
% erin EP1 -> data collection and power (why should I use this model?)
% erin --> wouldn't trust AI to do the job they already do;
% (?) authentictiy (?)
%   - kyrie mentions 'storytelling' to stay authentic; so hard for genAI to replicate her voice; being authentic!
%   - sasha --> passing off work that isn't your own
%   - somebody else! (who, someone) --> passing off work that isn't your own




% haylee: unclear boundaries from others:
% “I think I would feel embarrassed if anybody read my artist statement and was like, ‘Did you use ChatGPT for this?’” Haylee indicates that the social stigma surrounding use is still underdeveloped. She wrestles with the possible different reactions of peers to her using generative AI tools, “I think most people probably use it and would be like, that’s a tool you should use any tool at your disposal to help you convey your ideas.”

% Haylee: “I have less moral quandary with using AI for my business than I do my art stuff ‘cause the art stuff feels like a personal reflection of my intellect and the business stuff - It’s like, well, this is a business. … I have to participate in capitalism, so I don’t mind [getting] as much help as I can with that to make  money. I need to make a living wage, you know? But when it comes to my own artistic stuff, [there are some] ethical things around it that is hard.”









% ======== Thoughts ======== 
% evaluating output? do we need something here?
%   - evaluating output is hard; entreprenurs had different ways of doing it
%   - it's what I wanted (Bhavya)
%   - i already knew it (Haylee)
% ==========================


% ================ SPACE ? ? ? ========================
% \subsection{Entrepreneurs' and Providers' Insights for Design}

% \subsection{Supporting Various Modes for Engagement}
% In cases where entreprenuers and providers weren't implicated in shared use, they pointed out how systems which do share use could be helpful


% I think it's also important to note here that this is in isolation from other's shared use. Even when they did not see the possibility of shared use, when presented with the storyboards that were shared use they pointed out

%

% Alicia and/or Cella: shared use could be useful in ~'bridging the comfort gap' associated with these technologies

% Jarmele, who expereinced shared use at the workshops, notes how having online shared use can make her feel more comfortable to ask a question: GOOD QUOTE abt stupid questions
% 


% \subsubsection{Facilitating Exploration}
% To overcome operational barriers associated with using generative AI (e.g. prompting), entrepreneurs and providers suggested moving beyond chat interfaces. 
% LE1, describes that for those not comfortable with prompting, "big icons and like a small nudge will definitely help you a long way." EP1 pointed out how large icons, and buttons presses instead of prompting could help better "facilitate exploration and discovery" in a way that is easier than "the completely wide open world of like, enter whatever text you want to enter." 
% For LE2, large buttons to organize by different categories of her business , and while she keeps her current prompts in book with paper and pen.

% Some entrepreneurs had brief introduction to the technology at incubator, while other shared with their long-time friends and business partners. The comfort entrepreneurs had with others in their introduction and use to generative AI was often related to the extent they continued to use.

% Savion - small nudges go a long way (prompting as the biggest barrier)
% Alicia - facilitating exploration beyond chat interfaces
% general like of the panels
% Organization matches entreprenrial workflow, doing so many things; seperating tasks is important --- Jarmele

% \subsubsection{Meeting Entrepreneurs Where They Are At}
% Overall, entrepreneurs suggested that the medium for entrepreneurs to interact with generative AI be on platforms that they are already using (LE1, , LE7,
% Savion - slack
% Cella - facebook groups is popular
% Erin - signal for prototype
% 



==> Paper_Content/5_Discussion-OLD_.tex <==
% Aakash's advice:
% This is where the magic happens (for scholarly goals at least). This is the section where you distil your work, add your subjective evaluations, and push the field forward. This is subjective and an opportunity to push the field in the direction you want. This can be written in any way. But importantly, it has to do three things: (1) it has to be a stand alone section (many academics just read this), (2) address the "So what?" question (academic are often cynical about new work and certainly always skeptic so you need to do this well), and (3) acknowledge limitations and possibilities of future work/direction. 


% engage with other literature

\section{Implications for Design}
In this research, we sought to answer the questions: (RQ1) \textit{What aspects of these networks is helpful to sustain use of  generative AI technologies}? (RQ2) \textit{How can technology be designed to support social use of generative AI technologies?}. 
Here we discuss some key ideas. 
%First, we position our findings in the context of other social support models for local entrepreneurship. Then, a
%Acknowledging the inherent limitations within system design for addressing complex socio-technical problems~\cite{ackerman2000intellectual}, w
We situate the following implications as initial ideas for how designers may address the emergent socio-technical gaps in generative AI technologies and entrepreneurship~\cite{ackerman2000intellectual}.

\subsection{Meeting Entrepreneurs Where They Are At}
In responding to the \textit{''What''} across our storyboards (see Fig. \ref{fig:storyboard}), entrepreneurs expressed a diverse array of ways they would to prefer to engage with generative AI. While preferences across SMS, email, browser extensions were unclear, entrepreneurs and providers largely wanted to engage with generative AI systems not on proprietary platforms, but within existing systems they were already using. In response to S17, which featured a Facebook Group with ChatGPT in the mix, participants suggested their preferred social platform to engage on. For instance, for E1 this was Slack, P3 suggested Signal, and P2 agreed with Facebook. Given the variety of preferences across entrepreneurs, designing to meet entrepreneurs where they are at is an inherently difficult task.


\subsection{Beyond Chat Interfaces}
Consistent with literature we highlighted showing the difficulties with prompting \cite{}, local entrepreneurs in our study pointed out the continued difficulty that prompting (E1, E2, E5, P1, P2, P4) posed. By socially situating use E1, E2, and E5 ameliorated those difficulties or avoided them entirely (E5). Yet, prompting continues to be a challenge when interacting with generative AI, posing both a continued barrier to effectively using and discovering the capabilities of the technology. As P4 put it, they do not feel like \textit{''have the language to extract the most [they] can out of these programs''}. 
To overcome these barriers, E1 and P2 pointed out how S13, which featured large buttons for entrepreneurs to select categories to prompt in, could help \textit{''facilitate exploration''} (P2) and lower the barriers to prompting. E1 suggests that simple interface changes amounting to a \textit{''small nudge''} in the form of large buttons to obfuscate the prompting interaction method could go a long way in supporting use. P1 commented on how by organizing the interface in the targeted manner, you open up the opportunity for learning by passive exploration. By having interfaces where the barrier for exploration is clicking a button rather than formulating a prompt provides the potential to support entrepreneurs onboarding to generative while still learning digital literacies related to generative AI required by most systems (such as prompt generation).


% Prompting as (biggest operational barrier to usiung generative AI); Ariel doesn't feel like they have the langauge to get out 

% -----Took out because this is not novel --- we explained this in methods. ----
% \subsubsection{Centering Practicality}
% % Providing immediate value --> can't just be centered around discovery / open ended --> needs to provide immediate value;
% Providers shared how centering practicality is particularly important with local entrepreneurs given constrained resources, so when discovering potentially beneficial new technologies the goal should be centered around a practical outcome "instead of making a doodad" (P3).

% Bringing these reflections into system design, providers (P1, P2) indicated that gamified systems for generative AI education in the context of entrepreneurship breach this balance between discoverability and practicality by providing no immediate value to the entrepreneur, and in some cases replicating the "infantalizing nature" of certain participatory design practices (P1). 

\subsection{Dangers of Model-Based Solutions}
In response to storyboards highlighting model-centric solutions for local entrepreneurs, such as S18 and S19, which featured a model training off of entrepreneurs interactions with technical assistance providers to provide remote assistance, providers (P1, P2) and entrepreneurs (E2) emphatically opposed them, pointing out the potentially extractive nature of creating model-based solutions and its danger particularly with local entrepreneurs. 
While providers (P1, P2, P3) commented on the need for augmenting existing provider support systems, providers (P1, P2, P3) point out that there exists a larger question that preempts the creation of that model: What power do entrepreneurs give up by providing that data to the model? 

E2 commented on how the goals of the model, which are building context about the entrepreneur in order to support them, are largely achievable through low-tech interventions. 
Particularly, LE2 reflected on how she takes detailed notes when interacting with providers for support. 
Similarly, P1 and P2, who are both providers at the same entrepreneurial tech-assistance program, both pointed out how standardizing the note-taking to give entrepreneurs a starting point after appointments could largely replace what the model was trying to achieve.

% Supporting various modes of enagement comes from a reflection from all of this (dif social uses and preferences, dif preferences for meeting entreprenurs where they are at, dif ethical considerations using), so would not be suited for a findings contribution


% ---------------------------------


 

% In the end, entrepreneurs with richer continued social support systems supporting their use of generative AI tended to continue using the technology more.

% past work documents the resourcefulness of entreprenuers from lean economies. Can we build on that to put a narrative to how shared use of generative AI emerged as a function of keeping up with high cost of the technology, yet in turn, 

% ======== Socially constructed ideas of what is ok =======
% potential for social uses to establish more consensus in entreprenurial networks on which uses are ok
% 
% seeing what trusted peers are doing; coming to understanding and dialogue of what should be left to the generative AI what should be left to the human
% =========================================================



% ======== Yasmine Idea from 01/16/2024 meeting
% Problem: keeping up: this constant fear of wanting to keep up, not wanting to be left behind
%       - social media, keeping up with algorithmic design
% maybe if chatgpt was able to do the keep-up: here are the hashtags that you should be creating
% social media platforms to help entreprenuers better use generative AI 
%       - e.g. here's the latest prompt you need to try
% The Algorithm vs ChatGPT
% KEEPING UP IS HARD
% ============


% ====== Another Idea ======
% While a definition of digital literacy in the context of generative AI doesn't yet exist, it is clear that an entrepreneur needs to have an understanding of the capabilities of a generative AI system in order to understand how they may utilize it for their business. Discussion could contribute how they started to get this understanding 
% socially sitauted digital literacy in the context of generative AI.
% 
% 
% like, what even is/could be digital literacy for generative AI given this idea that models are black boxes?
% socially situated use of generative AI to facilitate building digital literacy?
% ==========================

% ====== Another Idea ======
% Postmodern social constructionist theory
% i.e. morals and ethics are socially constructed --> they inform a lot of use of generative AI, yet there remains gray areas, and in those cases entreprenuers look at what their peers think...
% supporting a menu of modes for engagement would allow for more construction of ethics for a network, which could better guide system design on navigating the boundaries for certain networks and in turn democratize the design of systems around use.
% people have varying levels of comfort and engagement
% well, this kind of already exists with like social media having generative AI content on it, that is a mode of engagement, though not a mode of use. 
% ==========================

\subsection{Limitations}
There were many limitations in this study.
First, the entrepreneurs recruited in this study were some of the most highly engaged in the two entrepreneurship hubs in which we focused our recruitment.
This could skew our results as highly engaged entrepreneurs within the entrepreneurial hub would be likely to have richer networks and more sustained support systems.
We attempted to account for this by including entrepreneurial support personnel from both community centers within our sample, to be able to speak on a wider range of entrepreneurs' experiences.
In addition, given the number of interviews and storyboards generated, the feedback on potential technological futures we received was inherently limited. 
We tried to account for this by presenting a range of storyboards, and iterate upon existing storyboards throughout the duration of the study.
Finally, this study was exploratory in nature, and we did not formally evaluate entrepreneurs sustained use of generative AI within their trusted networks and through shared accounts.
Rather, we provide the insights entrepreneurs provided while comparing their experiences to the scenarios displayed within storyboards, and from those make observations on how entrepreneurs sustained use.
